Stochastic Surprisal: An inferential measurement of Free Energy in Neural Networks

This paper conjectures and validates a framework that allows for action during inference in supervised neural networks. Supervised neural networks are constructed with the objective to maximize their performance metric in any given task. This is done by reducing free energy and its associated surprisal during training. However, the bottom-up inference nature of supervised networks is a passive process that renders them fallible to noise. In this paper, we provide a thorough background of supervised neural networks, both generative and discriminative, and discuss their functionality from the perspective of free energy principle. We then provide a framework for introducing action during inference. We introduce a new measurement called stochastic surprisal that is a function of the network, the input, and any possible action. This action can be any one of the outputs that the neural network has learnt, thereby lending stochasticity to the measurement. Stochastic surprisal is validated on two applications: Image Quality Assessment and Recognition under noisy conditions. We show that, while noise characteristics are ignored to make robust recognition, they are analyzed to estimate image quality scores. We apply stochastic surprisal on two applications, three datasets, and as a plug-in on twelve networks. In all, it provides a statistically significant increase among all measures. We conclude by discussing the implications of the proposed stochastic surprisal in other areas of cognitive psychology including expectancy-mismatch and abductive reasoning.

==> Sections/Old_Comments.tex <==
\begin{comment}

\section{Introduction}
\begin{figure}[tb]
 	\centering
 	\includegraphics[width=1\columnwidth]{Figs/New_Concept.png}
 	\caption{Perception and action in the physical world and its impact on the internal generative model.}\label{fig:Concept}
\end{figure}

\begin{itemize}
    \item We use ImageNet~\citep{deng2009imagenet} dataset as the underlying data used to train the deep learning model. For both the applications of saliency and IQA, the training phase will not use their specific datasets. For recognition, we will perform experiments on distorted CIFAR-10 images and we will not use the distorted images while training.
    \item The proposed technique is a \emph{plug-in} approach on top of a network. In both IQA and recognition experiments, we will show results on top of existing networks to show a performance improvement. On Saliency datasets, we show that recognition and object detection networks have implicit saliency comparable to those trained on large-scale gaze tracking datasets.
\end{itemize}


\begin{figure}[tb]
 	\centering
 	\includegraphics[width=1\columnwidth]{Figs/Concept.png}
 	\caption{Block diagram for Variational Autoencoder (VAE) and Sparse Autoencoder (SAE). The image $x$ is taken from the CURE-TSR dataset}\label{fig:Concept}
\end{figure}




This is similar to IQA where research has taken two directions. In this paper, we provide a definition that is scene and context dependent. We do so by utilizing the Free-energy principle~\citep{friston2009free} to define expectancy, and the mismatch. Consider Figure~\ref{fig:Concept}b. The challenge is to define an action in neural networks that would quantify surprisal. 

The contributions of this work are as follows:

\begin{itemize}
    \item Define Stochastic surprisal for every data point and provide a mathematical measure for stochastic surprisal. Generate stochastic surprisal as 
    \item Define Expectancy based on existing models and 
    \item IQA and Human Visual Saliency
\end{itemize}




A number of recent works that build on these psychological processes include emotion recognition~\cite{demekas2020investigation},.. . All these works argue for constructing \emph{better} internal generative models.~\emph{Better} is mathematically defined as minimizing the entropy of the generative model and hence its free energy. Entropy of any system is minimized by minimizing the occurrence of events which are atypical or \emph{surprising} as described in~\cite{buckley2017free}. However, the \emph{surprising} events are, by definition both unknown and unknowable, thereby creating a paradox for the system. This is got around by assuming that the system has a model of the outside world and the atypical input is interacting with this internal model and is a function of it which is tractable.

In this paper, we discuss the applications of Image Quality Assessment and Human Visual Saliency as functions of a system's internal generative model bounded by its Free-Energy.    


In this paper, we argue for constructing methods unifying image quality and assessment and recognition. In other words, we propose a concept that is able to assess the noise characteristics in images to assign objective quality as well as ignore the same noise characteristics to robustly classify images. Such a 

Free-energy principle is a documented and accepted principle in neuroscience that embodies the biological functioning of the brain. Simply put, the free energy principle states that a system minimizes its free energy to attain a state of equilibrium.

The idea that two separate applications must share a common set of applications is not new. Consider the 

Computationally, free energy principle is derived as an upper bound on the entropy of a probability distribution. Consider a neural network $f(\cdot)$ trained on a data distribution $\mathcal{X}$. In a classification setting, $f(\cdot)$ is trained to differentiate a given data point $x \in \mathcal{X}$ into one of $N$ classes. The inference can be considered in two stages. Mathematically, these are shown as, 

\begin{equation}
    \text{Free Energy} = \text{KL Divergence} + \text{Surprisal}
\end{equation}

Consider an $L$-layered network $f(\cdot)$ trained on a domain $X$ for a certain task. $f(\cdot)$ stores knowledge about the task on $X$ in the parameters of its layers - $W_l$ and $b_l$, $\forall l \in [1,L]$. Given an input image $x$, feed-forward inference projects the image on these parameters to make a decision $\hat{y}$. The projections are activations and are feed-forward features $y_{feat}^l$. For the task of classification, where $f(\cdot)$ is trained to classify between $N$ classes, the last layer is commonly a fully connected layer consisting of $N$ weights or filters. During inference the feed-forward features $y_{feat}^{L-1} = f_{L-1}(x)$, are projected independently onto each of the $N$ filters. The filter with the maximum projection is inferred as the class to which the image $x$ belongs. Mathematically, $y_{feat}^{L-1}$ and $\hat{y}$ are related as,



\begin{align}
    & y_{feat}^{L-1} = f_{L-1}(x), \label{eq:feature}\\
    \hat{y} = & \operatorname*{arg\,max} (W_L^T y_{feat}^{L-1} + b_L), \label{eq:Filter}\\
    \forall  W_L\in \Re^{d_{L-1}\times N}, & y_{feat}\in \Re^{d_{L-1}\times 1}, b_L\in \Re^{N\times 1}, 
\end{align}
where $W_L$ and $b_L$ are the parameters of the final fully connected layer. 

Logits are vectors of un-normalized predictions that are the outputs from the last layer of a neural network. These logits are fed to a softmax function that generates normalized probabilities with one value for each one of $N$ classes. The maximum probability is chosen as the class.

Softmax function is a common methodology of creating a probability distribution from $y^{L}$. Softmax probability distribution for logits $y$ is given by,

\begin{equation}
    \sigma(z)_i = \frac{e^z_i}{\sum_{j=1}^{N}e^z_j}
\end{equation}

System: A neural network $f(\cdot)$ trained on a distribution $\mathcal{X}$. A trained system that does not take in any external inputs to change or update its weights. We consider that a trained system is at NESS density.

Internal state of the system: $f_{\theta}^L(x|z)$.

External state of the world: $g_{\phi}(z|x)$.

Markov Blanket: $f_{\theta}^l(x|z)$.

However, the recent advancements in machine learning has extended the overton window of the utility of perception. Large scale datasets, like ImageNet and CURE-TSR. Neural networks have significantly outscaled. The creation of adversarial images and calibration issues depicts the inadequacy of the probability distribution using logits. Hence, a number of methods have been proposed to resolve this challenge.

A trained neural network's view of the Free-Energy Principle. 


The objective function that is optimized through Bayesian
inference is the surprisal (negative log probability) of sensory
data under a model. This quantifies the fit of the model to
the data (Schwartenbeck et al., 2015). The above suggests that
action and perception are both engaged in minimizing surprisal.
Interestingly, the average surprisal is the entropy alluded to
above. Minimizing the former on average corresponds to the
minimization of sensory entropy and ensures the occupancy of
a small number of highly probable states—i.e., self-organization.
While surprisal is a difficult quantity to directly assess, it is
bounded by a more tractable quantity: variational free energy.
As such, minimizing free energy ensures an upper bound on
surprisal and entropy

All living systems have a Markov blanket, because in order for
a system to be alive, it must be endowed with some degree of
conditional independence from its environment, or else it would
be indistinguishable from it

Given that the environment is only seen by agents through a
Markov blanket, an agent’s best bet at survival is to generate
probabilistic inferences about its environment via sensory signals.
In predictive coding formulations of free energy minimization,
this may proceed through generating predicted observations
(i.e., predicted sensory states) from an internal generative model
and comparing these to observed states. The results of this
comparison comprise a prediction error and can be thought of as
a simple form of free energy. These prediction errors can either
be used to update beliefs generating predictions (i.e., perception)
or they can be used to sample the environment in a way that
conforms to predictions (i.e., action) (Feldman, 2009). For an
accurate prediction of what the environment entails, the agent
must minimize free energy or prediction errors (Conant and
Ashby, 1991; Ashby, 1947; Conant and Ashby, 1970; Mansell,
2011; Solway and Botvinick, 2012). Mathematically, this is the
same as maximizing model evidence. In the context of machine
learning, this is equivalent to maximization of an evidence lower
bound or “ELBO” (Winn and Bishop, 2005

firstly, from a structural point of view, the supervised backpropagation of errors in a neural network only supports an implicit generative model, and thus the agent lacks explicit control of prior beliefs that are important in generating predictions of emotion. Second, in supervised learning, the objective function (the function that the algorithm aims to optimize) is a scalar function of an outcome, usually a classification of accuracy, rather than a functional of beliefs (Gan et al., 2017). This means that supervised learning models do not have an explicit or proper way to accommodate uncertainty, nor can have beliefs about the consequences of action. Thirdly, deep learning models never perform action to optimize belief updating all learning, and they are unable to actively elicit responses from their users.

For a single neuron, the blanket includes the presynaptic and postsynaptic membrane potentials that mediate its interactions with other neurons~\cite{hipolito2021markov}. In neural networks, these are the weight and bias connections. For cortical columns, the blanket will include neural populations mediating interactions between different columns. In principle, the identification of functional boundaries can proceed at finer (ion channels and molecules) and coarser (networks, brains, and people) scales.


Similarly, markov blankets in neural networks can be differentiated by the layers. The earlier layers are more sensitive to edges and colors while later layers are more conducive to abstract concepts. However, much like the brain these differentiating boundaries are not specific and while the overall scale is multiscale hierarchial. A number of blankets exist within the brain 

\section{Methods}

SAEs differ from VAEs in the loss function $J(x; \theta, \phi)$. For SAEs, we enforce latent space sparsity by using mean square error and elastic net regularization~\cite{zou2005regularization, prabhushankar2018semantically} for $\mathcal{L}$ and $\Omega$, respectively. The cost function for training our SAE is,
\begin{equation}
    J(x;\theta,\phi) = \lVert x -\tilde{x} \rVert_2^2 + \beta\lVert z_s \rVert_1 + \lambda\lVert \theta;\phi \rVert_2^2,
%\vspace{-1.5mm}
\end{equation}
where, $\theta$ and $\phi$ are the weight parameters for the encoder and decoder, respectively. $\beta=3$ and $\lambda=3e^{-3}$ are set as suggested by the authors in~\cite{ng2012ufldl}. The loss function of VAEs are defined as
\begin{equation}
    J(x;\theta, \phi) = - \mathbb{E}_{g_\phi(z|x)}[\log f_\theta(x | z)] + \text{KL}[g_\phi(z|x)|| f(z)].
\end{equation}
KL is the Kullback Leibler divergence between two distributions and we assume $f(z) = N(z| \textbf{0}, I)$. Thus, KL divergence constrains the latent space of VAEs to be a Gaussian distribution. The first term in the loss corresponds to the reconstruction error, $\mathcal{L}$, and the second term is a latent constraint, $\Omega$ in Eq.~(\ref{eq:loss}). In this paper, we use the trained representation spaces of both SAEs and VAEs to validate our methodology.
\vspace{-1.5mm}

The latent representation spaces $z_s$ and $z_g$ are low-dimensional manifolds embedded in a high dimensional input space. The activation of encoder is a projection of image on the learned manifold~\cite{Bengio2013}. The generalizability of autoencoder is ensured when test images are drawn from the same training distribution and are well projected in the vicinity of the learned manifold. However, the presence of distortions in test images causes their activations to move away from the representation manifold. Unless this movement is tangential to the manifold, the representations may not be accurate enough for the subsequent tasks. This limits the capability of activation from the encoder in characterizing the distortions in the input space. This is shown in Fig.~\ref{fig:manifold}, where both $x_1$ and $x_2$ have the same activation $x_{recon}$ on the manifold.

To alleviate this problem, we propose to utilize the gradients of trained autoencoder to characterize distortions in the test images. The geometric interpretation of backpropagated weight gradients is explained in subsection~\ref{subsec:Geometry}, while the gradient generation methodology is described in subsection~\ref{subsec:Gradient Generation}.

\begin{figure}[tb]
 	\centering
 	\includegraphics[width=.49\columnwidth]{Figs/manifold.pdf}
 	\vspace{-0.2cm}
 	\caption{Geometric visualization for gradients from test images.}\label{fig:manifold}
 	\vspace{-0.2cm}
\end{figure}
\begin{figure}[tb]
 	\centering
 	\includegraphics[width=.99\columnwidth]{Figs/GradGeneration.png}
 	\vspace{-0.2cm}
 	\caption{Block Diagram for gradient generation. The image $x$ is taken from the CURE-TSR dataset.}\label{fig:GradGen}
 	\vspace{-0.2cm}
\end{figure}

We make the following assumptions:
\begin{itemize}
    \item Presence of a trained internal model. We place no constraints on the nature of the model. Infact, we show that for both discriminative and generative models, our definition of stochastic surprisal holds.
    \item Presence of both original and distorted images for Image Quality Assessment. This falls under the Full-Reference Image Quality Assessment (FR-IQA) paradigm of quality assessment. While the concept discussed in this paper can be applied in a No-Reference Image Quality Assessment (NR-IQA) manner, where there is no requirement of distorted images, we do not do so here and only provide a discussion in Section.~\ref{subsec:Future}.
\end{itemize}

In Fig.~\ref{fig:manifold}, we visualize the geometric interpretation of gradients. We assume the manifold of reconstructed training images to be linear for the simplicity of explanation. As shown in the figure, the manifold of reconstructed training images is considered to be spanned by the weights of the encoder and the decoder. When the test images are the variations of training images, the autoencoder approximates the reconstruction, $x_{recon}$, by projecting them on the learned reconstructed training image manifold, $g_\phi (f_\theta (x))$. The gradient of weights can be calculated using the loss defined in Eq.~(\ref{eq:loss}) and the backpropgataion, $\frac{\partial J}{\partial \theta}, \frac{\partial J}{\partial \phi}$. These gradients represent required changes in the reconstructed image manifold to incorporate the test images. Therefore, we use these gradients to characterize the orthogonal distortions toward the test images. For instance, when $x_1$ and $x_2$ are projected onto different activations in the direction of the weight gradients $\frac{\partial J}{\partial \theta}, \frac{\partial J}{\partial \phi}$, they become distinguishable in the gradient space. We note that the assumption of linear manifold does not hold in most of practical scenarios but the geometric interpretation of gradients is still applicable to nonlinear manifolds. 

\end{comment}

==> Tables/Losses.tex <==
\begin{table}
\tiny
\centering
\caption{Analysis of $\mathcal{A}_d$ for ResNet-18 on CIFAR-10C.}
\begin{tabular}{l c c c c c c c c r} 
 \toprule
   Feed-Forward & MSE-M & CE & BCE & L1 & L1-M & Smooth L1 & Smooth L1-M & NLL & SoftMargin  \\ [0.5ex] 
 \midrule
   $67.89\%$ & $\textbf{71.4\%}$ & $69.47\%$ & $70.76\%$ & $70.12\%$ & $70.72\%$ & $70.42\%$ & $70.63\%$ & $70.93\%$ & $70.91\%$ \\ [1ex] 
 \midrule
\end{tabular}
\label{table:Losses}
\end{table}
\vspace{-3mm}

==> Tables/tab_IQA_All.tex <==
\begin{table*}[htb!]
\tiny

\centering
\caption{Overall performance of image quality estimators.}
\label{tab:iqa_results_all_before}


\begin{threeparttable}


\rotatebox{90}{\begin{tabular}{p{1.5cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{0.75cm}p{1cm}p{1cm}p{1.1cm}}
\hline

%\begin{tabular}{ccccccccccccccccccc} \hline


\multirow{3}{*}{{\bf Databases }}                 & \bf PSNR  &\bf SSIM  &\bf MS  &\bf CW &\bf IW  &\bf SR  &\bf FSIM  &\bf FSIMc  &\bf BRIS  & \bf BIQI &\bf BLII &\bf Per &\bf CSV &\bf UNI &\bf COHER &\bf SUM &\bf Proposed \\
&\bf HA & &\bf SSIM  &\bf SSIM  &\bf SSIM  &\bf SIM  & &&\bf QUE & &\bf NDS2 &\bf SIM & & \bf QUE & \bf ENSI & MER & \\ 
%&\cite{ponomarenko2011modified} & \cite{ponomarenko2011modified} &\cite{wang2004image} &\cite{wang2003multiscale} &\cite{sampat2009complex}&\cite{wang2011information}&\cite{zhang2012sr} &\cite{zhang2011fsim} &\cite{zhang2011fsim} &\cite{mittal2012no} &\cite{moorthy2010two} &\cite{saad2012blind}&\cite{temel2015persim} & \cite{Temel201692}&\cite{temel2016unique}  &\cite{Temel_SPIC_2018} &\cite{Temel_SPIC_2018} &
\\ \hline


 
               
%\textbf{\begin{tabular}[p]{@{}c@{}}Code source  \\ \end{tabular}}   & - &\cite{code_psnrhma}  &\cite{code_psnrhma}  &\cite{code_live}   &\cite{code_live}   &\cite{code_cwssim}   &\cite{code_iwssim}     &\cite{code_srsim}  &\cite{code_fsim}    & \cite{code_fsim}    &\cite{code_live}   &\cite{code_live}   &\cite{code_live}    & \cite{code_olives}    & \cite{code_olives}& \cite{code_olives}&\cite{code_olives} &\cite{code_olives} \\ 

%\textbf{\begin{tabular}[p]{@{}c@{}}Code version \\ \end{tabular}}   &-  &1.0  &1.0  &1.0   &-   &1.0   &-     &1.0  &1.0    & 1.0    &1.0   &1.0   &- & 1.0   &1.0 & 1.0& 1.0&1.0 \\ 

%\textbf{\begin{tabular}[p]{@{}c@{}}Copyright year \\ \end{tabular}}   & - &2011  &2011  &2009   &2003  &2010   &2011     &2011 &2010    & 2010    &2011   &2009   &2011    & 2015   &2016    & 2016& 2014&2017 \\ \hl
         
                & \multicolumn{17}{c}{\textbf{Outlier Ratio (OR, $\downarrow$)}}                                                                                                                                                                        \\ \hline
\textbf{MULTI}  
& 0.013 & 0.016 & 0.013 & 0.093 & 0.013 &\cellcolor{blue!10} \bf 0.000 & 0.018 & 0.016 & 0.067 & 0.024 & 0.078 & 0.004 &\cellcolor{blue!10} \bf 0.000 &\cellcolor{blue!10} \bf 0.000 & 0.031 &\cellcolor{blue!10} \bf 0.000 & \cellcolor{blue!10} \bf 0.000
\\                            
\textbf{TID13}  
&\cellcolor{blue!10} \bf 0.615 & 0.734 & 0.743 & 0.856 & 0.701 & 0.632 & 0.742 & 0.728 & 0.851 & 0.856 & 0.852 & 0.655 & 0.687 & 0.640 & 0.833 & \cellcolor{blue!10} \bf 0.620 & \cellcolor{blue!10} \bf 0.620
 \\ 
 \hline


               
               
                & \multicolumn{17}{c}{\textbf{Root Mean Square Error (RMSE, $\downarrow$)}}                                                                                                                                                                        \\ \hline


\textbf{MULTI}  
& 11.320 & 11.024 & 11.275 & 18.862 & 10.049 &\cellcolor{blue!10} \bf 8.686 & 10.866 & 10.794 & 15.058 & 12.744 & 17.419 & 9.898 & 9.895 & 9.258 & 14.806 & 8.212 & \cellcolor{blue!10} \bf 7.943\\


\textbf{TID13}    & 0.652 & 0.762 & 0.702 & 1.207 & 0.688 &\cellcolor{blue!10} \bf 0.619 & 0.710 & 0.687 & 1.100 & 1.108 & 1.092 & 0.643 & 0.647 & 0.615 & 1.049  & 0.630 & \cellcolor{blue!10} \bf 0.596
 \\ \hline
             
               
               & \multicolumn{17}{c}{\textbf{Pearson Linear Correlation Coefficient (PLCC, $\uparrow$)}}                                                                                                                                                                        \\ \hline 
               
 
\multirow{2}{*}{{\bf MULTI}}                                  
& 0.801 & 0.813 & 0.803 & 0.380 & 0.847 & 0.888 & 0.818 & 0.821 & 0.605 & 0.739 & 0.389 & 0.852 & 0.852 &  0.872 & 0.622 &\cellcolor{blue!10} \bf  0.901 & \cellcolor{blue!10} \bf 0.908 \\                                          
& -1 & -1 & -1 & -1 & -1 & 0 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & 0 & 

 \\


\multirow{2}{*}{{\bf TID13}}                               
& 0.851 & 0.789 & 0.830 & 0.227 & 0.832 & 0.866 & 0.820 & 0.832 & 0.461 & 0.449 & 0.473 & 0.855 & 0.853 & \cellcolor{blue!10} \bf 0.869 & 0.533  &  0.861 & \cellcolor{blue!10} \bf 0.877\\
& -1 & -1 & -1 & -1 & -1 & 0 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & 0 & -1 & -1 & 
   \\ \hline







\textbf{}      & \multicolumn{17}{c}{\textbf{Spearman's Rank Correlation Coefficient (SRCC, $\uparrow$)}}                                                                                                                                                                        \\ \hline   

       
\multirow{2}{*}{{\bf MULTI}}                                          
& 0.715 & 0.860 & 0.836 & 0.631 & \cellcolor{blue!10} \bf 0.884 & 0.867 & 0.864 & 0.867 & 0.598 & 0.611 & 0.386 & 0.818 & 0.849 &  0.867 & 0.554  & \cellcolor{blue!10} \bf 0.884 & \cellcolor{blue!10} \bf 0.887 \\   
& -1 & 0 & -1 & -1 & 0 & 0 & 0 & 0 & -1 & -1 & -1 & -1 & -1 & 0 & -1 & 0 & 
\\
 
  
\multirow{2}{*}{{\bf TID13}}
& 0.847 & 0.742 & 0.786 & 0.563 & 0.778 & 0.807 & 0.802 & 0.851 & 0.414 & 0.393 & 0.396 &0.854 & 0.846 & \cellcolor{blue!10} \bf 0.860 & 0.649  & 0.856 & \cellcolor{blue!10} \bf 0.865 \\

& -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & -1 & 0 & -1 & 0 & -1 & 0 & 


  \\ \hline
      
 
 
 
\textbf{}      & \multicolumn{17}{c}{\textbf{Kendall's Rank Correlation Coefficient (KRCC, $\uparrow$)}}                                                                                                                                                                        \\ \hline    


\multirow{2}{*}{{\bf MULTI}}                                              
& 0.532 & 0.669 & 0.644 & 0.457 & \cellcolor{blue!10} \bf 0.702 & 0.678 & 0.673 & 0.677 & 0.420 & 0.440 & 0.268 & 0.624 & 0.655 &  0.679 & 0.399 & 0.698 & \cellcolor{blue!10} \bf 0.702\\                                         

& -1 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & -1 & -1 & -1 & -1 & 0 & 0 & -1 & 0 & 

 \\  

\multirow{2}{*}{{\bf TID13}}                                          
& 0.666 & 0.559 & 0.605 & 0.404 & 0.598 & 0.641 & 0.629 & 0.667 & 0.286 & 0.270 & 0.277 &\cellcolor{blue!10} \bf 0.678 & 0.654 & 0.667 & 0.474   & 0.667 & \cellcolor{blue!10} \bf 0.677 \\
& 0 & -1 & -1 & -1 & -1 & -1 & -1 & 0 & -1 & -1 & -1 & 0 & 0 & 0 & -1 & 0 & 
\\ \hline
\end{tabular}
}
\end{threeparttable}
\vspace{-0.5cm}
\end{table*}

==> Tables/tab_IQA_subset.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{table}[t!]
\tiny

\centering
\caption{Performance of proposed Stochastic Surprisal based UNIQUE against other Image Quality Estimators. Top 2 results in each row are highlighted.}
\label{tab:iqa_results_subset}




%\begin{tabular}{||p{0.55cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.55cm}|p{0.50cm}p{0.7cm}||}
\begin{tabular}{c c c c c c c c c c}
\hline

%\begin{tabular}{ccccccccccccccccccc} \hline


\multirow{3}{*}{{\bf Database }} & \bf PSNR  &\bf IW  &\bf SR &\bf FSIMc &\bf Per &\bf CSV &\bf SUM &\bf UNIQUE &\bf Stochastic\\
&\bf HA &\bf SSIM  &\bf SIM  & &\bf SIM & & \bf MER & \bf & & Surprisal  \\ %&\cite{ponomarenko2011modified} &\cite{wang2011information} &\cite{zhang2012sr} & \cite{zhang2011fsim} &\cite{temel2015persim} & \citet{Temel201692} &\citet{Temel_SPIC_2018} &\citet{temel2016unique} &
%\\ \hline

                & \multicolumn{9}{c}{\textbf{Outlier Ratio (OR, $\downarrow$)}}                                                                                                                                                                        \\ \hline
\textbf{MULTI}  
& 0.013 & 0.013 & \bf 0.000 & 0.016 & 0.004 & \bf 0.000 & \bf 0.000 & \bf 0.000 &  \bf 0.000
\\                            
\textbf{TID13}  
& \bf 0.615 & 0.701 & 0.632 & 0.728 & 0.655 & 0.687 & \bf 0.620 & 0.640 &  \bf 0.620
 \\ 
 \hline
               
                & \multicolumn{9}{c}{\textbf{Root Mean Square Error (RMSE, $\downarrow$)}}                                                                                                                                                                        \\ \hline

\textbf{MULTI}  
& 11.320 & 10.049 & 8.686 & 10.794 & 9.898 & 9.895 & \bf 8.212 & 9.258 &  \bf 7.943\\


\textbf{TID13}    & 0.652 & 0.688 & 0.619 & 0.687 & 0.643 & 0.647 & 0.630 & \bf 0.615 &  \bf 0.596
 \\ \hline
             
               & \multicolumn{9}{c}{\textbf{Pearson Linear Correlation Coefficient (PLCC, $\uparrow$)}}                                                                                                                                                                        \\ \hline 
               
\multirow{2}{*}{{\bf MULTI}}                                  
& 0.801 & 0.847 & 0.888 & 0.821 & 0.852 & 0.852 & \bf 0.901 &  0.872 &  \bf 0.908 \\                                          
& -1 & -1 & 0 & -1 & -1 & -1 & -1 & -1 & \\

\multirow{2}{*}{{\bf TID13}}                               
& 0.851 & 0.832 & 0.866 & 0.832 & 0.855 & 0.853 & 0.861 & \bf 0.869 &  \bf 0.877\\
& -1 & -1 & 0 & -1 & -1 & -1 & 0 & 0 & 
   \\ \hline

\textbf{}      & \multicolumn{9}{c}{\textbf{Spearman's Rank Correlation Coefficient (SRCC, $\uparrow$)}}                                                                                                                                                                        \\ \hline   

\multirow{2}{*}{{\bf MULTI}}                                          
& 0.715 & \bf 0.884 & 0.867 & 0.867 & 0.818 & 0.849 & \bf 0.884 &  0.867 &  \bf 0.887 \\   
& -1 & 0 & 0 & 0 & -1 & -1 & 0 & 0 & 
\\
 
  
\multirow{2}{*}{{\bf TID13}}
& 0.847 & 0.778 & 0.807 &0.851 & 0.854 & 0.846 &  0.856 & \bf 0.860 &  \bf 0.865 \\

& -1 & -1 & -1 & -1 & 0 & -1 & 0 & 0 & 


  \\ \hline
      
 
 
 
\textbf{}      & \multicolumn{9}{c}{\textbf{Kendall's Rank Correlation Coefficient (KRCC)}}                                                                                                                                                                        \\ \hline    


\multirow{2}{*}{{\bf MULTI}}                                              
& 0.532 &  \bf 0.702 & 0.678 & 0.677 & 0.624 & 0.655 &  0.698 & 0.679 &  \bf 0.702\\                                         

& -1 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 

 \\  

\multirow{2}{*}{{\bf TID13}}                                          
& 0.666 & 0.598 & 0.641 & 0.667 & \bf 0.678 & 0.654 & 0.667 & 0.667 & \bf 0.677 \\
& 0 & -1 & -1 & 0 & 0 & 0 & 0 & 0 & 
\\ \hline
\end{tabular}

%\end{threeparttable}
\end{table}

==> Tables/tab_saliency.tex <==
\begin{table*}[!tp]
\small
\centering
\caption{Robustness Analysis of Implicit Saliency}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{} &
\multicolumn{5}{c|}{NSS} &
\multicolumn{5}{c|}{CC} \\
\hline
 Gaussian &Sal&Deep&ML&Shallow&\textbf{Implicit} &Sal&Deep&ML&Shallow&\textbf{Implicit}\\ [0ex] 
 Blur   &Gan&GazeII&Net&Deep&\textbf{Saliency} &Gan&GazeII&Net&Deep&\textbf{Saliency}\\ [0ex] 
\hline
$r=0$ & $0.8977$ & $0.6214$ & $0.5431$ &$\mathbf{0.9306}$&$0.7981$ & $\mathbf{0.6280}$ & $0.5927$ &$0.4481$&$0.5120$ &$0.4051$\\
\hline
$r=50$ & $\downarrow0.2239$ & $\downarrow0.3436$ &$\downarrow0.2484$ &$\downarrow0.2025$& $\mathbf{\downarrow0.1793}$&$\downarrow0.2731$ &$\downarrow0.3954$ &$\downarrow0.2940$&$\downarrow0.1840$&$\mathbf{\downarrow0.1432}$ \\
\hline

\end{tabular}
\label{table:NSS and CC result}
\end{table*}
